Position Paper: Bridging the Gap Between Machine Learning and Sensitivity Analysis

We argue that interpretations of machine learning (ML) models or the model-building process can be seen as a form of sensitivity analysis (SA), a general methodology used to explain complex systems in many fields such as environmental modeling, engineering, or economics. We address both researchers and practitioners, calling attention to the benefits of a unified SA-based view of explanations in ML and the necessity to fully credit related work. We bridge the gap between both fields by formally describing how (a) the ML process is a system suitable for SA, (b) how existing ML interpretation methods relate to this perspective, and (c) how other SA techniques could be applied to ML.

==> latex-math/ml-ensembles.tex <==
% ml - bagging, random forest
\newcommand{\bl}[1][m]{b^{[#1]}} % baselearner, default m
\newcommand{\blh}[1][m]{\hat{b}^{[#1]}} % estimated base learner, default m 
\newcommand{\blx}[1][m]{b^{[#1]}(\xv)} % baselearner, default m
\newcommand{\fM}{f^{[M]}(\xv)} % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(\xv)} % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)} % ambiguity/instability of ensemble
\newcommand{\betam}[1][m]{\beta^{[#1]}} % weight of basemodel m
\newcommand{\betamh}[1][m]{\hat{\beta}^{[#1]}} % weight of basemodel m with hat
\newcommand{\betaM}{\beta^{[M]}} % last baselearner

% ml - boosting
\newcommand{\fm}[1][m]{f^{[#1]}} % prediction in iteration m
\newcommand{\fmh}[1][m]{\hat{f}^{[#1]}} % prediction in iteration m
\newcommand{\fmd}[1][m]{f^{[#1-1]}} % prediction m-1
\newcommand{\fmdh}[1][m]{\hat{f}^{[#1-1]}} % prediction m-1
\newcommand{\errm}[1][m]{\text{err}^{[#1]}} % weighted in-sample misclassification rate
\newcommand{\wm}[1][m]{w^{[#1]}} % weight vector of basemodel m
\newcommand{\wmi}[1][m]{w^{[#1](i)}} % weight of obs i of basemodel m
\newcommand{\thetam}[1][m]{\thetab^{[#1]}} % parameters of basemodel m
\newcommand{\thetamh}[1][m]{\hat{\thetab}^{[#1]}} % parameters of basemodel m with hat
\newcommand{\blxt}[1][m]{b(\xv, \thetab^{[#1]})} % baselearner, default m
\newcommand{\ens}{\sum_{m=1}^M \betam \blxt} % ensemble
\newcommand{\rmm}[1][m]{\tilde{r}^{[#1]}} % pseudo residuals
\newcommand{\rmi}[1][m]{\tilde{r}^{[#1](i)}} % pseudo residuals
\newcommand{\Rtm}[1][m]{R_{t}^{[#1]}} % terminal-region
\newcommand{\Tm}[1][m]{T^{[#1]}} % terminal-region
\newcommand{\ctm}[1][m]{c_t^{[#1]}} % mean, terminal-regions
\newcommand{\ctmh}[1][m]{\hat{c}_t^{[#1]}} % mean, terminal-regions with hat
\newcommand{\ctmt}[1][m]{\tilde{c}_t^{[#1]}} % mean, terminal-regions
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-eval.tex <==
% resampling
\newcommand{\ntest}{n_{\mathrm{test}}} % size of the test set
\newcommand{\ntrain}{n_{\mathrm{train}}} % size of the train set
\newcommand{\ntesti}[1][i]{n_{\mathrm{test},#1}} % size of the i-th test set
\newcommand{\ntraini}[1][i]{n_{\mathrm{train},#1}} % size of the i-th train set
\newcommand{\Jtrain}{J_\mathrm{train}} % index vector train data
\newcommand{\Jtest}{J_\mathrm{test}} % index vector test data
\newcommand{\Jtraini}[1][i]{J_{\mathrm{train},#1}} % index vector i-th train dataset
\newcommand{\Jtesti}[1][i]{J_{\mathrm{test},#1}} % index vector i-th test dataset
\newcommand{\Dtraini}[1][i]{\mathcal{D}_{\text{train},#1}} % D_train,i, i-th training set
\newcommand{\Dtesti}[1][i]{\mathcal{D}_{\text{test},#1}} % D_test,i, i-th test set

\newcommand{\JSpace}[1][m]{\nset^{#1}} % space of train indices of size n_train
\newcommand{\JtrainSpace}{\nset^{\ntrain}} % space of train indices of size n_train
\newcommand{\JtestSpace}{\nset^{\ntest}} % space of train indices of size n_test
\newcommand{\yJ}[1][J]{\yv_{#1}} % output vector associated to index J
\newcommand{\yJDef}{\left(y^{(J^{(1)})},\dots,y^{(J^{(m)})}\right)} % def of the output vector associated to index J
\newcommand{\JJ}{\mathcal{J}} % cali-J, set of all splits
\newcommand{\JJset}{\left((\Jtraini[1], \Jtesti[1]),\dots,(\Jtraini[B], \Jtesti[B])\right)} % (Jtrain_1,Jtest_1) ...(Jtrain_B,Jtest_B)
\newcommand{\Itrainlam}{\ind(\Dtrain, \lamv)}
% Generalization error
\newcommand{\GE}{\mathrm{GE}} % GE
\newcommand{\GEh}{\widehat{\GE}} % GE-hat 
\newcommand{\GEfull}[1][\ntrain]{\GE(\ind, \lamv, #1, \rho)} % GE full
\newcommand{\GEhholdout}{\GEh_{\Jtrain, \Jtest}(\ind, \lamv, |\Jtrain|, \rho)} % GE hat holdout
\newcommand{\GEhholdouti}[1][i]{\GEh_{\Jtraini[#1], \Jtesti[#1]}(\ind, \lamv, |\Jtraini[#1]|, \rho)} % GE hat holdout i-th set
\newcommand{\GEhlam}{\GEh(\lamv)} % GE-hat(lam) 
\newcommand{\GEhlamsubIJrho}{\GEh_{\ind, \JJ, \rho}(\lamv)} % GE-hat_I,J,rho(lam) 
\newcommand{\GEhresa}{\GEh(\ind, \JJ, \rho, \lamv)} % GE-hat_I,J,rho(lam) 
\newcommand{\GErhoDef}{\lim_{\ntest\rightarrow\infty} \E_{\Dtrain,\Dtest \sim \Pxy} \left[ \rho\left(\yv_{\Jtest}, \FJtestftrain\right)\right]} % GE formal def
\newcommand{\agr}{\mathrm{agr}} % aggregate function
\newcommand{\GEf}{\GE\left(\fh\right)} % GE of a fitted model
\newcommand{\GEfh}{\GEh\left(\fh\right)} % GEh of a fitted model
\newcommand{\GEfL}{\GE\left(\fh, L\right)} % GE of a fitted model wrt loss L
\newcommand{\Lyfhx}{L\left(y, \hat{f}(\xv)\right)} % pointwise loss of fitted model
\newcommand{\GEnf}[1]{GE_n\left(\fh_{#1}\right)} % GE of a fitted model
\newcommand{\GEind}{GE_n\left(\ind_{L, O}\right)} % GE of inducer
\newcommand{\GED}{\GE_{\D}} % GE indexed with data
\newcommand{\EGEn}{EGE_n} % expected GE
\newcommand{\EDn}{\E_{|D| = n}} % expectation wrt data of size n

% performance measure
\newcommand{\rhoL}{\rho_L} % perf. measure derived from pointwise loss
\newcommand{\F}{\boldsymbol{F}} % matrix of prediction scores
\newcommand{\Fi}[1][i]{\F^{(#1)}} % i-th row vector of the predscore mat
\newcommand{\FJ}[1][J]{\F_{#1}} % predscore mat idxvec J 
\newcommand{\FJf}{\FJ[J,f]} % predscore mat idxvec J and model f
\newcommand{\FJtestfh}{\FJ[\Jtest, \fh]} % predscore mat idxvec Jtest and model f hat
\newcommand{\FJtestftrain}{\F_{\Jtest, \Itrainlam}} % predscore mat idxvec Jtest and model f
\newcommand{\FJtestftraini}[1][i]{\F_{\Jtesti[#1],\ind(\Dtraini[#1], \lamv)}}  % predscore mat i-th idxvec Jtest and model f
\newcommand{\FJfDef}{\left(f(\xv^{(J^{(1)})}),\dots, f(\xv^{(J^{(m)})})\right)} % def of predscore mat idxvec J and model f
\newcommand{\preimageRho}{\bigcup_{m\in\N}\left(\Yspace^m\times\R^{m\times g}\right)} % Set of all datasets times HP space

% ml - ROC
\newcommand{\np}{n_{+}} % no. of positive instances
\newcommand{\nn}{n_{-}} % no. of negative instances
\newcommand{\rn}{\pi_{-}} % proportion negative instances
\newcommand{\rp}{\pi_{+}} % proportion negative instances
  % true/false pos/neg:
\newcommand{\tp}{\# \text{TP}} % true pos
\newcommand{\fap}{\# \text{FP}} % false pos (fp taken for partial derivs)
\newcommand{\tn}{\# \text{TN}} % true neg
\newcommand{\fan}{\# \text{FN}} % false neg

==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax} % IGNORE_NOTATION


==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\fvec}{\left[f\left(\xi[1]\right), \dots, f\left(\xi[n]\right) \right]} % function vector
\newcommand{\fv}{\mathbf{f}} % function vector
\newcommand{\kv}{\mathbf{k}} % cov matrix partition
\newcommand{\kxxp}{k\left(\xv, \xv^{\prime} \right)} % cov of x, x'
\newcommand{\kxij}[2]{k\left(\xi, \xi[j] \right)} % cov of x_i, x_j
\newcommand{\mv}{\mathbf{m}} % GP mean vector
\newcommand{\Kmat}{\mathbf{K}} % GP cov matrix
\newcommand{\gaussmk}{\normal(\mv, \Kmat)} % Gaussian w/ mean vec, cov mat
\newcommand{\gp}{\mathcal{GP}\left(m(\xv), \kxxp \right)} % Gaussian Process Definition
\newcommand{\ls}{\ell} % length-scale
\newcommand{\sqexpkernel}{\exp \left(- \frac{\| \xv - \xv^{\prime} \|^2}{2 \ls^2} \right)} % squared exponential kernel

% GP prediction
\newcommand{\fstarvec}{\left[f\left(\xi[1]_{\ast}\right), \dots, f\left(\xi[m]_{\ast}\right) \right]} % pred function vector
\newcommand{\kstar}{\kv_{\ast}} % cov of new obs with x
\newcommand{\kstarstar}{\kv_{\ast \ast}} % cov of new obs
\newcommand{\Kstar}{\Kmat_{\ast}} % cov mat of new obs with x
\newcommand{\Kstarstar}{\Kmat_{\ast \ast}} % cov mat of new obs
\newcommand{\preddistsingle}{f_{\ast} ~|~ \xv_{\ast}, \Xmat, \fv} % predictive distribution for single pred
\newcommand{\preddistdefsingle}{\normal(\kstar^{T}\Kmat^{-1}\fv, \kstarstar - \kstar^T \Kmat ^{-1}\kstar)} % Gaussian distribution for single pred
\newcommand{\preddist}{f_{\ast} ~|~ \Xmat_{\ast}, \Xmat, \fv} % predictive distribution
\newcommand{\preddistdef}{\normal(\Kstar^{T}\Kmat^{-1}\fv, \Kstarstar - \Kstar^T \Kmat ^{-1}\Kstar)} % Gaussian predictive distribution


==> latex-math/ml-infotheory.tex <==
% basic info theory
\newcommand{\entx}{- \sum_{x \in \Xspace} p(x) \cdot \log p(x)} % entropy of x
\newcommand{\dentx}{- \int_{\Xspace} f(x) \cdot \log f(x) dx} % diff entropy of x
\newcommand{\jentxy}{- \sum_{x \in \Xspace} p(x, y) \cdot \log p(x, y)} % joint entropy of x, y
\newcommand{\jdentxy}{- \int_{\Xspace, \Yspace} f(x, y) \cdot \log f(x, y) dx dy} % joint diff entropy of x, y
\newcommand{\centyx}{- \sum_{x \in \Xspace} p(x) \sum_{y \in \Yspace} p(y|x) \cdot \log p(y|x)} % cond entropy y|x
\newcommand{\cdentyx}{- \int_{\Xspace, \Yspace} f(x, y) \cdot \log f(y | x) dx dy} % cond diff entropy y|x
\newcommand{\xentpq}{- \sum_{x \in \Xspace} p(x) \cdot \log q(x)} % cross-entropy of p, q
\newcommand{\kldpq}{D_{KL}(p \| q)} % KLD between p and q
\newcommand{\kldpqt}{D_{KL}(p \| q_{\thetab})} % KLD divergence between p and parameterized q
\newcommand{\explogpq}{\E_p \left[\log \frac{p(X)}{q(X)} \right]} % expected LLR of p, q (def KLD)
\newcommand{\sumlogpq}{\sum_{x \in \Xspace} p(x) \cdot \log \frac{p(x)}{q(x)}} % expected LLR of p, q (def KLD)

==> latex-math/ml-interpretable.tex <==
%%%%%% perturbed data
\usepackage{xifthen}
\newcommand{\pert}[3]{\ifthenelse{\equal{#2}{}}{\tilde{#1}}{\ifthenelse{\equal{#3}{}}{\tilde{#1}^{#2}}{\tilde{#1}^{#2|#3}}}}	% command to express that for #1 the subset #2 was perturbed given subset #3

%%%%%% marginalized functions
\newcommand{\fj}{f_j} % marginal function f_j, depending on feature j
\newcommand{\fnj}{f_{-j}} % marginal function f_{-j}, depending on all features but j
\newcommand{\fS}{f_S} % marginal function f_S depending on feature set S
\newcommand{\fC}{f_C} % marginal function f_C depending on feature set C
\newcommand{\fhj}{\fh_j} % marginal function fh_j, depending on feature j
\newcommand{\fhnj}{\fh_{-j}} % marginal function fh_{-j}, depending on all features but j
\newcommand{\fhS}{\fh_S} % marginal function fh_S depending on feature set S
\newcommand{\fhC}{\fh_C} % marginal function fh_C depending on feature set C
\newcommand{\XSmat}{\Xmat_S} % Design matrix subset
\newcommand{\XCmat}{\Xmat_C} % Design matrix subset
\newcommand{\Xnj}{\Xmat_{-j}} % Design matrix subset -j = {1, .., j-1, j+1, ..., p}

%%%%% Shapley values
\newcommand{\Scupj}{S \cup \{j\}} % coalition S but without player j
\newcommand{\Scupk}{S \cup \{k\}} % coalition S but without player k
\newcommand{\SsubP}{S \subseteq P} % coalition S subset of P
\newcommand{\SsubPnoj}{\SsubP \setminus \{j\}} % coalition S subset of P without player j
\newcommand{\SsubPnojk}{\SsubP \setminus \{j,k\}} % coalition S subset of P without player k
\newcommand{\phiij}{\hat{\phi}_j^{(i)}} % Shapley value for feature j and observation i

%%%%% LIME 
\newcommand{\Gspace}{\mathcal{G}} % Hypothesis space for surrogate model
\newcommand{\neigh}{\phi_{\xv}} % Proximity measure
\newcommand{\zv}{\mathbf{z}} % Sampled datapoints for surrogate
\newcommand{\Zspace}{\mathcal{Z}} % Space of sampled datapoints
\newcommand{\Gower}{d_G} % Gower distance



==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons
\newcommand{\hidz}{\mathbf{z}}  % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}} % bias vector
\newcommand{\biasc}{c} % bias in output
\newcommand{\wtw}{\mathbf{w}} % weight vector (general)
\newcommand{\Wmat}{\mathbf{W}} % weight vector (general)
\newcommand{\wtu}{\mathbf{u}} % weight vector of output neuron

% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)} % regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)} % unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)} % penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)} % regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)} % unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)} % unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)} % unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)} % optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)} % dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))} % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))} % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))} % undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))} % denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}} % ??
\newcommand{\Ci}[1][i]{C^{(#1)}} % ??  
\newcommand{\oi}[1][i]{o^{(#1)}} % ??  
\newcommand{\ti}[1][i]{t^{(#1)}} % ??  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% linear svm
\newcommand{\sv}{\operatorname{SV}} % supportvectors
\renewcommand{\sl}{\zeta} % slack variable
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)} % slack variable vector
\newcommand{\sli}[1][i]{\zeta^{(#1)}} % i-th slack variable
\newcommand{\scptxi}{\scp{\thetab}{\xi}} % scalar prodct of theta and xi
\newcommand{\svmhplane}{\yi \left( \scp{\thetab}{\xi} + \theta_0 \right)} % SVM hyperplane (normalized)
\newcommand{\alphah}{\hat{\alpha}} % alpha-hat (basis fun coefficients)
\newcommand{\alphav}{\bm{\alpha}} % vector alpha (bold) (basis fun coefficients)
\newcommand{\alphavh}{\hat{\bm{\alpha}}} % vector alpha-hat (basis fun coefficients)
\newcommand{\dualobj}{\sumin \alpha_i - \frac{1}{2}\sumin \sumjn \alpha_i\alpha_j\yi \yi[j] \scp{\xi}{\xv^{(j)}}} % min objective in lin svm dual

% nonlinear svm
\newcommand{\HS}{\Phi} % H, hilbertspace
\newcommand{\phix}{\phi(\xv)} % feature map x
\newcommand{\phixt}{\phi(\tilde \xv)} % feature map x tilde
\newcommand{\kxxt}{k(\xv, \tilde \xv)} % kernel fun x, x tilde
\newcommand{\scptxifm}{\scp{\thetab}{\phi(\xi)}} % scalar prodct of theta and xi


==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}} % (Parent) node N
\newcommand{\Npk}{\Np_k} % node N_k
\newcommand{\Nl}{\Np_1}	% Left node N_1
\newcommand{\Nr}{\Np_2} % Right node N_2
\newcommand{\pikN}[1][k]{\pi_#1^{(\Np)}} % class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}} % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}} % estimated class probability left node
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}} % estimated class probability right node

